Search Improves Label for Active Learning

We investigate active learning with access to two distinct oracles: Label (which is standard) and Search (which is not). The Search oracle models the situation where a human searches a database to seed or counterexample an existing solution. Search is stronger than Label while being natural to implement in many situations. We show that an algorithm using both oracles can provide exponentially large problem-dependent improvements over Label alone.

==> unionofintervalsbad.tex <==
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
% User Packages:
% 
% 
\psscalebox{1.0 1.0} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-2.775)(10.2,2.775)
\psline[linecolor=black, linewidth=0.04, arrowsize=0.05291666666666667cm 2.0,arrowlength=1.4,arrowinset=0.0]{<-}(0.8,2.825)(0.8,-2.375)(10.0,-2.375)
\psline[linecolor=black, linewidth=0.04](0.8,-0.375)(1.6,-0.375)
\psline[linecolor=black, linewidth=0.04](1.6,1.225)(2.4,1.225)
\psline[linecolor=black, linewidth=0.04](2.4,-2.375)(3.2,-2.375)(3.2,-2.375)(3.2,-2.375)
\psline[linecolor=black, linewidth=0.04](3.2,-0.375)(4.0,-0.375)
\psline[linecolor=black, linewidth=0.04](4.0,1.225)(5.6,1.225)
\psline[linecolor=black, linewidth=0.04](5.6,-0.375)(8.8,-0.375)
\rput[bl](0.4,-0.375){$0.5$}
\rput[bl](0.4,1.225){$1$}
\rput[bl](0.0,2.425){$\eta(x)$}
\rput[bl](10.0,-2.775){$x$}
\rput[bl](0.4,-2.375){$0$}
\rput[bl](1.2,-2.775){$0.1$}
\rput[bl](2.0,-2.775){$0.2$}
\rput[bl](2.8,-2.775){$0.3$}
\rput[bl](3.6,-2.775){$0.4$}
\rput[bl](5.6,-2.775){$0.6$}
\rput[bl](8.8,-2.775){$1$}
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm](1.6,1.225)(1.6,-0.375)(1.6,-0.375)
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm](2.4,1.225)(2.4,-2.375)
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm](3.2,-2.375)(3.2,-0.375)
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm](4.0,-0.375)(4.0,1.225)
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm](5.6,1.225)(5.6,-0.375)(5.6,-0.375)
\end{pspicture}
}


